From Learner Behavior to Reusable Skills for Effective and Efficient Learner Simulation

Learner simulation aims to reproduce how a particular learner behaves on new tasks. Although Large Language Models (LLMs) can generate increasingly fine-grained learning behaviors, existing approaches often need to repeatedly process a growing interaction history to reconstruct the learner. This introduces additional context and inference costs and makes the acquired learner-specific simulation capability difficult to reuse across different LLMs. We therefore propose Learner2Skill, which externalizes the simulation capability acquired from historical interactions into a persistent and reusable Simulation Skill. The Skill captures the learner's current learning state and recurring response patterns, evolves as new real interactions arrive, and can be adapted to a new LLM through lightweight executor calibration without reconstructing the learner from scratch. Experiments show that Learner2Skill more faithfully reproduces fine-grained learner behavior while reducing overall token cost, and that the same constructed Skills can be effectively reused across different LLM executors.

==> sections/acknowledge.tex <==
\section{Acknowledgment}

We would like to thank the anonymous reviewers for their constructive feedback and the members of our test group for their valuable insights. Special thanks go to the LaTeX community for developing the tools and packages that made this project possible. Additionally, we extend our gratitude to Qwen and DeepSeek for their invaluable contributions to the development of this template. Their expertise in natural language processing and code generation greatly accelerated the project timeline and ensured the highest level of quality.


==> sections/discussions.tex <==
\vspace{-2mm}
\section{Discussions}

While our template addresses many challenges associated with arXiv submissions, several limitations remain. First, some advanced LaTeX users may prefer more granular control over formatting than our template currently offers. Second, although we aimed for broad compatibility, certain edge cases—such as highly specialized equation rendering—may require additional adjustments.

Future work could focus on expanding the template's feature set, integrating support for alternative markup languages (e.g., Markdown), and exploring machine learning techniques to automate parts of the formatting process. Continued collaboration with AI models like Qwen and DeepSeek will be crucial in realizing these advancements.
